Exploring the Influence of Driving Context on Lateral Driving Style Preferences: A Simulator-Based Study

Technological advancements focus on developing comfortable and acceptable driving characteristics in autonomous vehicles. Present driving functions predominantly possess predefined parameters, and there is no universally accepted driving style for autonomous vehicles. While driving may be technically safe and the likelihood of road accidents is reduced, passengers may still feel insecure due to a mismatch in driving styles between the human and the autonomous system. Incorporating driving style preferences into automated vehicles enhances acceptance, reduces uncertainty, and poses the opportunity to expedite their adoption. Despite the increased research focus on driving styles, there remains a need for comprehensive studies investigating how variations in the driving context impact the assessment of automated driving functions. Therefore, this work evaluates lateral driving style preferences for autonomous vehicles on rural roads, considering different weather and traffic situations. A controlled study was conducted with a variety of German participants utilizing a high-fidelity driving simulator. The subjects experienced four different driving styles, including mimicking of their own driving behavior under two weather conditions. A notable preference for a more passive driving style became evident based on statistical analyses of participants' responses during and after the drives. This study could not confirm the hypothesis that subjects prefer to be driven by mimicking their own driving behavior. Furthermore, the study illustrated that weather conditions and oncoming traffic substantially influence the perceived comfort during autonomous rides. The gathered dataset is openly accessible at https://www.kaggle.com/datasets/jhaselberger/idcld-subject-study-on-driving-style-preferences.

==> sections/methodology/method_lit_references.tex <==
\subsection{Lit References for Methodology}


==> sections/results/multi_regression.tex <==
\subsection{Hierarchical Linear Multiple Regression Model}

Building upon the preceding findings, a hierarchical linear multiple regression model was designed to examine the distinct relationships of individual variables in predicting on-drive relaxation levels.
As an initial step, age and gender were included as sociodemographic covariates.
The subsequent stage incorporates details about the subjects' driving style by including the six \ac{mdsi} factor scores.
For the third step, the driving context, including road section type, weather, and traffic situation, was incorporated into the model.
Finally, in the fourth step, the autonomous driving style was introduced.
The model and the obtained results are summarized in \autoref{tab:multiRegressionModel}.
Following that, an examination of the individual contributions of each variable type was conducted.
Variables were included in the regression model only if they significantly correlated with the dependent variable in the previous step.
Subsequently, the significant increment of $R^2$ in each step, along with the assessment of the \ac{aic} \cite{washington2020statistical}, was analyzed.
While $R^2$ is standardized and includes a significance test, according to \cite{ali2019hazard}, the \ac{aic} has the advantage of considering independent variable contributions and model complexity.
A lower AIC value indicates a better model fit.
With an $R^2$ of \num{0.24} and resulting Cohen's $f^2$ \cite{cohen2013statistical} effect size of \num{0.32}, the effect can be considered medium to strong.
Additionally, the \ac{aic} consistently decreased at each step compared to the previous one.
Results indicated that the AVs and the subjects' driving styles contributed the most to the observed variance in on-drive relaxation levels with a $\Delta R^2$ of \num{0.11} and \num{0.09}, followed by the driving context ($\Delta R^2 = 0.02$). 
As indicated by the previous evaluations, the switch from a passive to a sportive driving style in this model resulted in a significant decrease in the perceived relaxation \hlmregBetaPL{-0.90}.
The weather condition \hlmregBeta{-0.08}{.03} turned out to be the weakest predictor among the other driving context variables concerning the traffic situation\hlmregBetaPL{-0.19} and road segment type \hlmregBetaPL{-0.13}.

\input{tables/multiRegression.tex}

==> sections/results/self_assessment.tex <==
\subsection{Driving Style Self-Assessment}
To compare the self-assessment of the subjects' driving styles with the ratings on the \ac{arca}, \ac{tia}, and the on-drive relaxation questionnaires in the first step, the factor scores are calculated based on the MDSI questionnaire.
\autoref{tab:mdsi_de} in the Appendix presents the statistics of the subjects' responses and the internal consistency values (Cronbach's alpha) for the current sample.
Given the limited number of subjects in this study, which is considered insufficient for a substantial factor analysis of the MDSI items, the factor divisions and loadings are adopted from \cite{van2015measuring}.
Recent studies also report evidence indicating that the original eight driving styles of the MDSI can be condensed to six \cite{nees2021relationships, long2019reliability, padilla2020adaptation, trogolo2020factor, holman2015romanian}.
This version of the MDSI is also applied in \cite{van2018relation,haselberger2023self}.
To overcome the limited discriminatory capabilities of non-refined methods like Sum Scores by Factor or Weighted Sum Scores, similar to \cite{van2015measuring, karjanto2017identification, nees2021relationships}, refined scores are used by the multiple regression approach, which maximizes the validity of the estimates \cite{distefano2009understanding}. 
This method provides factor scores that indicate each subject's deviation from a factor's mean \cite{andy2009discovering}.
A person is assigned a high factor score when their score surpasses the average of all participants within that specific factor.
The factor with the highest average determines the driving style class. 
% The resulting refined, gender-specific distribution of the MDSI driving styles is visualized in \autoref{fig:mdsiRefindedStyleDistribution}.

% \begin{figure}[t]
%     \centering
% %    \frame{
%     \includegraphics[page=1,trim={0cm 0 0 0}, clip,width=0.5\linewidth]{assets/sim/MDSI_DS_Distribution.pdf}
% %    }
%     \caption{Relative distribution of subjects' driving styles determined from the MDSI questionnaire divided into women and men.}
%     \label{fig:mdsiRefindedStyleDistribution}
% \end{figure} 

==> tables/arcaItems.tex <==
\begin{table}[h]
    \caption{Used items and abbreviations of the \acf{arca} in English and German including the lower and upper bounds.}
    \centering
    \scriptsize
    % \begin{tabular}{llll}
    \begin{xltabular}{1\linewidth}{l >{\arraybackslash}X ll}
        \toprule
        \textbf{Abbreviation}   & \textbf{Item}                                                             & \textbf{lower} & \textbf{upper} \\
        \midrule
        Vehicle Control         & Vehicle control appeared \dots .                                               & unnatural            & natural              \\
                                & \textit{Die Fahrzeugsteuerung wirkte auf mich \dots .}                                    & \textit{unnatürlich}          & \textit{natürlich}            \\
        Stress Level            & Automated driving made me feel \dots .                                          & stressed             & relaxed              \\
                                & \textit{Ich fühlte mich während der Fahrt \dots .}                                      & \textit{beunruhigt}           & \textit{entspannt}            \\
        Behavior Predictability & I could … predict the vehicle's behavior.                                 & hardly               & easily               \\
                                & \textit{Ich konnte das Fahrzeugverhalten \dots vorhersagen.}                           & \textit{schwer}               & \textit{leicht}               \\
        Ride Comfort            & All in all, the automated ride was \dots .                                      & uncomfortable        & comfortable          \\
                                & \textit{Ich empfand das Fahrzeugverhalten insgesamt als \dots .}                         & \textit{unkomfortabel}        & \textit{komfortabel}          \\
        Satisfaction            & I am … with the way the automation controlled the vehicle.                & unhappy              & happy                \\
                                & \textit{Ich bin mit der Art und Weise, wie das Fahrzeug gefahren ist, insgesamt \dots .} & \textit{unzufrieden}          & \textit{zufrieden}            \\
                                \bottomrule
        % \end{tabular}
    \end{xltabular}
\label{tab:arcaItems}
\end{table}


==> tables/ds_estimates.tex <==
\begingroup

\setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.5} % Default value: 1


\begin{table}[h]
    \caption{Overlap of subject estimation and actual driving style divided into the two weather situations. The most significant total overlap in highlighted bold, weather-specific predominant class is underlined.}
    \centering
    \scriptsize
    \begin{tabular}{lllcccc}
        \toprule
        \textbf{}                & \textbf{}        & \textbf{} & \multicolumn{4}{c}{\textbf{Proportion Correct Estimates in \%}}              \\ \cline{4-7}\clineSpacing 
        \textbf{Driving   Style} & \textbf{Weather} & \textbf{} & \textbf{Passive} & \textbf{Rail} & \textbf{Replay} & \textbf{Sportive} \\
        \midrule
        Passive                  & Dry              &           & 31.3          & \underline{56.3}       & 9.4          & 3.1            \\
                                 & Rain             &           & \underline{59.4}          & 25.0       & 6.3          & 6.3            \\
                                 & Total            &           & \textbf{45.3}          & 40.6       & 7.8          & 4.7            \\
                                 &                  &           &                  &               &                 &                   \\
        Rail                     & Dry              &           & 28.1          & 25.0       & 15.6         & \underline{31.3}           \\
                                 & Rain             &           & \underline{40.6}          & 31.3       & 21.9         & 6.3            \\
                                 & Total            &           & \textbf{34.4}         & 28.1       & 18.8         & 18.8           \\
                                 &                  &           &                  &               &                 &                   \\
        Replay                   & Dry              &           & 3.1           & 6.3        & 37.5         & \underline{53.1}           \\
                                 & Rain             &           & 25.0          & 3.1        & \underline{59.4}         & 12.5           \\
                                 & Total            &           & 14.1          & 4.7        & \textbf{48.4}         & 32.8           \\
                                 &                  &           &                  &               &                 &                   \\
        Sportive                 & Dry              &           & 0.0           & 0.0        & 9.4          & \underline{90.6}           \\
                                 & Rain             &           & 18.8          & 3.1        & 9.4          & \underline{68.8}           \\
                                 & Total            &           & 9.4           & 1.6        & 9.4          & \textbf{79.7}          \\
                                 \bottomrule
        \end{tabular}
\label{tab:dsEstimates}
\end{table}


\endgroup

==> tables/mdsi_de.tex <==
\afterpage{
\onecolumn
\scriptsize
\renewcommand{\doublerulesep}{0pt}
\begin{xltabular}{1\linewidth}{l >{\arraybackslash}X cc}
%\caption{\small{\textsc{Summary of all MDSI related questions divided into the eight factors including statistics and reliability. The factor assignments are initially inherited from \cite{van2015measuring} and gradually enriched with remaining items from \cite{taubmann2004}, \cite{poo2013reliability}, and self-defined items. Participants scored their agreement on each item using a 6-point Likert scale, ranging from 1 (not at all) to 6 (very much).}}} \\
\caption{
    Summary the MDSI-DE \cite{haselberger2023self} questions divided into the eight factors including statistics and reliability. Participants scored their agreement on each item using a 6-point Likert scale, ranging from 1 (not at all) to 6 (very much).} \\
\toprule
\multicolumn{2}{l}{\textbf{MDSI items}} & \textbf{M} & \textbf{SD} \\
\midrule
\endfirsthead
\toprule
\multicolumn{2}{l}{\textbf{MDSI items}} & \textbf{M} & \textbf{SD} \\ 
\midrule
\endhead
\midrule
\multicolumn{4}{c}{\textit{Continued on next page\ldots}}\\
\endfoot
% \hline\hline
\endlastfoot
% &  &  &  \\
\multicolumn{2}{l}{\textbf{Factor 1 - Angry Driving (Cronbach's alpha 0.823)}} & \textbf{} & \textbf{} \\
43 & Honk my horn at others & 2.34 & 1.234 \\
3 & Blow my horn or "flash" the car in front as a way of expressing frustrations & 2.38 & 1.212 \\
28 & When someone does something on the road that annoys me, I   flash them with high beam & 2.31 & 1.533 \\
12 & Swear at other drivers & 3.59 & 1.316 \\
17 & When a traffic light turns green and the car in front of me doesn’t get going immediately, I try to urge the driver to move on & 3.22 & 1.338 \\
13 & When a traffic light turns green and the car in front of me   doesn’t get going, I wait for a while until it moves {[}-{]} & 4.53 & 1.367 \\
2 & Purposely tailgate other drivers & 2.44 & 1.243 \\
45 & Arguing with other drivers or pedestrians & 1.47 & 0.621 \\
46 & Get angry with people driving slow in the fast lane & 4.72 & 1.170 \\


 &  &  &  \\


\multicolumn{2}{l}{\textbf{Factor 2 - Risky Driving (Cronbach's alpha 0.897)}} & \textbf{} & \textbf{} \\
44 & Enjoy the excitement of dangerous driving & 2.59 & 1.316 \\
22 & Like to take risks while driving & 2.66 & 1.181 \\
24 & Like the thrill of flirting with death or disaster & 2.16 & 1.221 \\
6 & Enjoy the sensation of driving on the limit & 3.06 & 1.605 \\
29 & Get a thrill out of breaking the law & 1.66 & 0.937 \\
47 & Enjoy the power of the engine & 3.81 & 1.655 \\
48 & Enjoy shifting gears quickly & 3.25 & 1.566 \\
49 & Feel the car asking for more speed & 2.56 & 1.564 \\
50 & Drive faster when a vehicle is trying to pass me & 1.75 & 1.136 \\
51 & I enjoy the variation on curvy roads & 4.44 & 1.190 \\


 &  &  &  \\


\multicolumn{2}{l}{\textbf{Factor 3 - Anxious Driving (Cronbach's alpha 0.711)}} & \textbf{} & \textbf{} \\
31 & Feel nervous while driving & 1.69 & 0.965 \\
10 & Driving makes me feel frustrated & 2.13 & 1.157 \\
40 & Feel comfortable while driving {[}-{]} & 5.19 & 0.592 \\
4 & Feel I have control over driving {[}-{]} & 5.47 & 0.507 \\
25 & It worries me when driving in bad weather & 2.06 & 1.190 \\
33 & Feel distressed while driving & 1.50 & 0.950 \\
41 & Always ready to react to unexpected manoeuvres by other drivers {[}-{]} & 5.13 & 0.793 \\
8 & While driving, I try to relax myself {[}-{]} & 4.22 & 1.237 \\
52 & Driving on narrow rural roads overwhelms me & 1.84 & 0.920 \\


  &  &  &  \\


\multicolumn{2}{l}{\textbf{Factor 4 - Dissociative Driving (Cronbach's alpha 0.738)}} & \textbf{} & \textbf{} \\
35 & Attempt to drive away from traffic lights in third gear (or on   the neutral mode in automatic cars) & 1.16 & 0.369 \\
27 & Forget that my lights are on full beam until flashed by   another motorist & 1.94 & 0.914 \\
39 & Nearly hit something due to misjudging my gap in a parking   lot & 2.00 & 0.916 \\
36 & Plan my route badly, so that I hit traffic that I could have   avoided & 2.66 & 1.234 \\
34 & Intend to switch on the windscreen wipers, but switch on the   lights instead & 1.50 & 0.803 \\
20 & Fix my hair / makeup while driving & 1.25 & 0.880 \\
21 & Distracted or preoccupied, and suddenly realize the vehicle ahead has slowed down, and have to slam on the breaks to avoid a collision & 2.25 & 1.164 \\
5 & Drive through traffic lights that have just turned red & 1.88 & 0.871 \\
19 & When someone tries to skirt in front of me on the road, I   drive in an assertive way in order to prevent it & 2.41 & 1.192 \\
30 & Misjudge the speed of an oncoming vehicle when passing & 2.25 & 0.984 \\
15 & Lost in thoughts or distracted, I fail to notice someone at   the pedestrian crossings & 1.81 & 0.780 \\


 &  &  &  \\


\multicolumn{2}{l}{\textbf{Factor 5 - Careful Driving (Cronbach's alpha 0.685)}} & \textbf{} & \textbf{} \\
42 & Tend to drive cautiously & 4.06 & 1.190 \\
14 & Drive cautiously & 4.69 & 1.091 \\
23 & Base my behavior on the motto "better safe than   sorry" & 4.50 & 1.218 \\
7 & On a clear freeway, I usually drive at or a little below the   speed limit & 3.75 & 1.849 \\
41 & Always ready to react to unexpected maneuvers by other   drivers & 5.13 & 0.793 \\
53 & Wait patiently when not having right of way & 3.38 & 1.264 \\
54 & Wait patiently when you cannot advance the traffic & 4.56 & 1.243 \\


 &  &  &  \\


\multicolumn{2}{l}{\textbf{Factor 6 - Distress - Reduction Driving Style (Cronbach's alpha 0.371)}} & \textbf{} & \textbf{} \\
1 & Do relaxing activities while driving & 2.22 & 1.338 \\
37 & Use muscle relaxation techniques while driving & 1.59 & 1.043 \\
26 & Meditate while driving & 1.16 & 0.574 \\
11 & I daydream to pass the time while driving & 2.75 & 1.524 \\
55 & Listen to music to relax while driving & 4.69 & 1.306 \\
56 & Enjoy the landscape while driving & 3.88 & 1.238 \\
57 & If time permits, I prefer to drive on the rural road instead of the highway & 2.81 & 1.635 \\


 &  &  &  \\


\multicolumn{2}{l}{\textbf{Factor 7 - High-Velocity Driving Style (Cronbach's alpha 0.666)}} & \textbf{} & \textbf{} \\
16 & In a traffic jam, I think about ways to get through the   traffic faster & 3.50 & 1.503 \\
9 & When in a traffic jam and the lane next to me starts to move,   I try to move into that lane as soon as possible & 2.28 & 1.250 \\
17 & When a traffic light turns green and the car in front of me doesn’t get going immediately, I try to urge the driver to move on & 3.22 & 1.338 \\
2 & Purposely tailgate other drivers & 2.44 & 1.243 \\
32 & Get impatient during rush hours & 3.69 & 1.230 \\
5 & Drive through traffic lights that have just turned red & 1.88 & 0.871 \\

 &  &  &  \\


\multicolumn{2}{l}{\textbf{Factor 8 - Patient Driving Style (Cronbach's alpha 0.467)}} & \textbf{} & \textbf{} \\
18 & At an intersection where I have to give right-of-way to   oncoming traffic, I wait patiently for cross-traffic to pass & 5.22 & 0.975 \\
23 & Base my behaviour on the motto "better safe than sorry" & 4.50 & 1.218 \\
13 & When a traffic light turns green and the car in front of me   doesn’t get going, I wait for a while until it moves {[}-{]} & 4.53 & 1.367 \\
38 & Plan long journeys in advance & 2.50 & 1.481 \\


\bottomrule
\multicolumn{4}{l}{{[}-{]} reversed item} \\
\label{tab:mdsi_de}
\end{xltabular}
\twocolumn
}

==> tables/multiRegression.tex <==
\begingroup

\setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.5} % Default value: 1
\begin{table}[t]
    \caption{Hierarchical multiple regression predicting the on-drive relaxation level, $R^2 = 0.24,~p<.001$.}
    \centering
    \scriptsize
    
    \begin{tabular}{lccccc}
        \toprule
        \textbf{}                                     & $B$ & $SE$ & $\beta$ & $\Delta R^2$ & $AIC$ \\
        \midrule
        \textit{\textbf{Step 1 – Sociodemographic}}   &            &             &               & 0.01\pLevelThree         & 6391         \\
        ~~~$F(2,2037) = 12.5, p<.001$            &            &             &               &                   &              \\
                                                    %   &            &             &               &                   &              \\
        Age                                           & -0.02    & 0.01     & \tsHelper-0.11\pLevelThree    &                   &              \\
        Gender   (1=Female, 2 = Male)                 & -0.07    & 0.06     & -0.06       &                   &              \\
                                                      &            &             &               &                   &              \\
        \textit{\textbf{Step 2 - MDSI Factor Scores}} &            &             &               & 0.09\pLevelThree         & 6197         \\
        ~~~$F(8,2031)   = 30.4, p<.001$          &            &             &               &                   &              \\
        Age                                           & -0.03    & 0.01     & \tsHelper-0.16\pLevelThree   &                   &              \\
        Gender   (1=Female, 2 = Male)                 & 0.41     & 0.08     & \tsHelperP0.36\pLevelThree    &                   &              \\
        Angry                                         & -0.20    & 0.03     & \tsHelper-0.16\pLevelThree   &                   &              \\
        Risky                                         & -0.29    & 0.04     & \tsHelper-0.24\pLevelThree   &                   &              \\
        Anxious                                       & -0.38    & 0.04     & \tsHelper-0.29\pLevelThree   &                   &              \\
        Dissociative                                  & 0.40     & 0.05     & \tsHelper0.30\pLevelThree    &                   &              \\
        Careful                                       & -0.19    & 0.04     & \tsHelper-0.15\pLevelThree   &                   &              \\
        Distress                                      & 0.01     & 0.04     & ~~0.01       &                   &              \\
                                                      &            &             &               &                   &              \\
        \textit{\textbf{Step 3 - Driving Context}}  &            &             &               & 0.02\pLevelThree         & 6168         \\
        ~~~$F(11,2028)   = 25.6, p<.001$         &            &             &               &                   &              \\
        Age                                           & -0.03    & 0.01     & \tsHelper-0.16\pLevelThree   &                   &              \\
        Gender   (1=Female, 2 = Male)                 & 0.41     & 0.08     & \tsHelperP0.36\pLevelThree    &                   &              \\
        Angry                                         & -0.20    & 0.03     & \tsHelper-0.16\pLevelThree   &                   &              \\
        Risky                                         & -0.29    & 0.04      & \tsHelper-0.24\pLevelThree    &                   &              \\
        Anxious                                       & -0.38    & 0.04     & \tsHelper-0.29\pLevelThree   &                   &              \\
        Dissociative                                  & 0.40     & 0.05     & \tsHelperP0.30\pLevelThree    &                   &              \\
        Careful                                       & -0.19    & 0.04     & \tsHelper-0.15\pLevelThree   &                   &              \\
        Distress                                      & 0.01     & 0.04     & ~~0.01       &                   &              \\
        Road (1=Straight, 2=Curve)                    & -0.15    & 0.05     & \tsHelper-0.13\pLevelTwo~    &                   &              \\
        Weather (1=Dry, 2=Rain)                       & -0.10    & 0.05     & \tsHelper-0.09\pLevelOne~~     &                   &              \\
        Traffic (1=Clear, 2 = Oncoming)               & -0.22    & 0.05     & \tsHelper-0.19\pLevelThree   &                   &              \\
                                                      &            &             &               &                   &              \\
        \textit{\textbf{Step 4 - AV Driving Style}}   &            &             &               & 0.11\pLevelThree         & 5890         \\
        ~~~$F(14,2025) = 44.7, p<.001$           &            &             &               &                   &              \\
        Age                                           & -0.03     & 0.01     & \tsHelper-0.17\pLevelThree    &                   &              \\
        Gender (1=Female, 2 = Male)                   & 0.42      & 0.07     & \tsHelperP0.36\pLevelThree     &                   &              \\
        Angry                                         & -0.20    & 0.03     & \tsHelper-0.15\pLevelThree    &                   &              \\
        Risky                                         & -0.30    & 0.04     & \tsHelper-0.24\pLevelThree    &                   &              \\
        Anxious                                       & -0.38    & 0.03     & \tsHelper-0.29\pLevelThree    &                   &              \\
        Dissociative                                  & 0.39     & 0.04     & \tsHelperP0.30\pLevelThree      &                   &              \\
        Careful                                       & -0.19    & 0.03      & \tsHelper-0.15\pLevelThree      &                   &              \\
        Distress                                      & 0.02     & 0.04     & ~~0.013        &                   &              \\
        Road (1=Straight, 2=Curve)                    & -0.15    & 0.05      & \tsHelper-0.13\pLevelThree    &                   &              \\
        Weather (1=Dry, 2=Rain)                       & -0.10    & 0.05      & \tsHelper-0.08\pLevelOne~~       &                   &              \\
        Traffic (1=Clear, 2 = Oncoming)               & -0.22    & 0.05      & \tsHelper-0.19\pLevelThree     &                   &              \\
        Style (1 = Passive, 2 = Rail)                 & -0.22    & 0.06     & \tsHelper-0.19\pLevelThree    &                   &              \\
        Style (1 = Passive, 2 = Replay)               & -0.52    & 0.06     & \tsHelper-0.45\pLevelThree    &                   &              \\
        Style (1 = Passive, 2 = Sportive)             & -1.05    & 0.06     & \tsHelper-0.90\pLevelThree    &                   &              \\
        \bottomrule 
        \multicolumn{6}{l}{\footnotesize{Note: \pLevelOne~$p<.05$, \pLevelTwo~$p<.01$, \pLevelThree~$p<.001$}} \\
        \end{tabular}

\label{tab:multiRegressionModel}
\end{table}
\endgroup



==> tables/relaxResponsesMDSI.tex <==
\begingroup

\setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.5} % Default value: 1

\begin{table}[h]
    \caption{
        Marginal mean relaxation levels for the AV's four driving styles passive, rail, replay, and sportive grouped by the six MDSI driving styles careful, dissociative, angry, risky, anxious, and distress reduction.
        For MDSI style, the mean relaxation responses of the groups were analyzed with regard to their statistically significant differences using robust ANOVAs. The group differences were significant across all six MDSI driving styles, with \pValuePL.
        The superscript depicts the driving style of the AV for which there is a significant ($p<.05$) difference according to the post-hoc tests.
        }
    \centering
    \scriptsize
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{}         & \textbf{Careful}          & \textbf{Dissociative}    & \textbf{Angry}             & \textbf{Risky}               & \textbf{Anxious}             & \textbf{Distress} \\
        \midrule
        Passive (${P}$)   & 1.59 $\pm$ 0.79$^{S}$     & 1.40 $\pm$ 0.77$^{S}$    & 1.58 $\pm$ 0.63$^{Re,S}$   & 1.32 $\pm$ 0.90$^{R,Re,S}$   & 1.25 $\pm$ 0.79$^{Re,S}$     & 0.43 $\pm$ 1.06$^{S}$      \\
        Rail (${R}$)      & 1.33 $\pm$ 1.07$^{S}$     & 1.23 $\pm$ 0.95$^{S}$    & 1.14 $\pm$ 0.98$^{S}$      & 1.01 $\pm$ 1.03$^{S}$        & 1.17 $\pm$ 0.88$^{Re,S}$     & 0.64 $\pm$ 0.98$^{S}$      \\
        Replay (${Re}$)   & 1.37 $\pm$ 0.88$^{S}$     & 1.15 $\pm$ 0.98          & 0.63 $\pm$ 1.32            & 0.59 $\pm$ 1.33$^{S}$        & 0.44 $\pm$ 1.22              & 0.31 $\pm$ 0.89$^{S}$      \\
        Sportive (${S}$)  & 0.35 $\pm$ 1.28           & 0.838 $\pm$ 0.95         & 0.51 $\pm$ 1.32            & 0.17 $\pm$ 1.35              & -0.19 $\pm$ 1.27             & -0.30 $\pm$ 0.81     \\
        \bottomrule
        \end{tabular}


\label{tab:relaxResponsesMDSI}
\end{table}

\endgroup

==> tables/tiaItems.tex <==
\begin{table}[h]
    \caption{Used items and abbreviations of the \acf{tia} in English and German.}
    \centering
    \scriptsize
    \begin{tabular}{ll}
        \toprule
        \textbf{Abbreviation} & \textbf{Item}                                                             \\
        \midrule
        Situation Assessment  & The system is capable of interpreting situations correctly.               \\
                              & \textit{Das System ist imstande Situationen richtig einzuschätzen.}                \\
        System State          & The system state was always clear to me.                                  \\
                              & \textit{Mir war durchgehend klar, in welchem Zustand sich das System befindet.}    \\
        System Familiarity    & I already know similar systems.                                           \\
                              & \textit{Ich kenne bereits ähnliche Systeme.}                                       \\
        Trust in Developers   & The developers are trustworthy.                                           \\
                              & \textit{Die Entwickler sind vertrauenswürdig. }                                    \\
        Beware of System      & One should be careful with unfamiliar automated systems.                  \\
                              & \textit{Bei unbekannten automatisierten Systemen sollte man eher vorsichtig sein.} \\
        System Reliability    & The system works reliably.                                                \\
                              & \textit{Das System arbeitet zuverlässig.}                                          \\
        System Predictability & The system reacts unpredictably.                                          \\
                              & \textit{Das System reagiert unvorhersehbar.}                                       \\
        User Wellbeing        & The developers take my well-being seriously.                              \\
                              & \textit{Die Entwickler nehmen mein Wohlergehen ernst.}                             \\
        Trust in System       & I trust the system.                                                       \\
                              & \textit{Ich vertraue dem System.}                                                  \\
        System Failure        & A system malfunction is likely.                                           \\
                              & \textit{Ein Ausfall des Systems ist wahrscheinlich.}                 \\
        \bottomrule             
        \end{tabular}
\label{tab:tiaItems}
\end{table}

